Iterative Methods for Private Synthetic Data: Unifying Framework and New Methods

We study private synthetic data generation for query release, where the goal is to construct a sanitized version of a sensitive dataset, subject to differential privacy, that approximately preserves the answers to a large collection of statistical queries. We first present an algorithmic framework that unifies a long line of iterative algorithms in the literature. Under this framework, we propose two new methods. The first method, private entropy projection (PEP), can be viewed as an advanced variant of MWEM that adaptively reuses past query measurements to boost accuracy. Our second method, generative networks with the exponential mechanism (GEM), circumvents computational bottlenecks in algorithms such as MWEM and PEP by optimizing over generative models parameterized by neural networks, which capture a rich family of distributions while enabling fast gradient-based optimization. We demonstrate that PEP and GEM empirically outperform existing algorithms. Furthermore, we show that GEM nicely incorporates prior information from public data while overcoming limitations of PMW^Pub, the existing state-of-the-art method that also leverages public data.

==> checklist.tex <==
\section{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    Yes.
  \item Did you describe the limitations of your work?
    Yes.
  \item Did you discuss any potential negative societal impacts of your work?
    Yes.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    Yes.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    Yes.
	\item Did you include complete proofs of all theoretical results?
    Yes.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    Yes
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    Yes.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    Yes.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    Yes.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    Yes
  \item Did you mention the license of the assets?
    Not applicable.
  \item Did you include any new assets either in the supplemental material or as a URL?
    Yes. We submitted code in supplemental material.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    Not applicable
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    Not applicable
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    Not applicable.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    Not applicable.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    Not applicable.
\end{enumerate}

\end{enumerate}

==> docs/unused/ITER.tex <==
\subsection{\pep Update Oracle. }
% \textbf{ Changing to unnormalized distributions}

% \begin{itemize}
%     \item Try the query projection algorithm from \cite{nikolov2013geometry} with the Iterative projection protocol. That is first the the noisy answers $\widetilde{q(\Dprivbf)} = q(\Dprivbf) + \text{Gaussian}(\rho)$. Then use IP to find a dataset that matches the answers $\widetilde{q(\Dprivbf)}$.
% \end{itemize}

%
%
%%%%%%%%%%%%%%%%%
%% Claim
%%%%%%%%%%%%%%%%%
% \begin{claim}\label{claim:I}
% For any query set $Q$.
% Let  $\Dbf$ be a distribution that can be expressed as $D(x) = \frac{U(x)}{Z} \exp\pp{\sum_{q\in Q}\lambda_q q(x)}$ for all $x$, and $\Pbf$ is any distribution then
% \begin{align*}
%     \sum_{x\in \cX} P(x) \log\pp{\frac{D(x)}{U(x)}} = \sum_{q\in Q} \lambda_q q(\Pbf) - \log(Z)
% \end{align*}
% \end{claim}
% \begin{proof}
% \begin{align*}
%     \sum_{x\in \cX} P(x) \log\pp{\frac{D(x)}{U(x)}}
%     = \sum_{x\in \cX} P(x) \pp{\sum_{q\in Q}\lambda_q q(x)} - \log(Z)
%     = \sum_{q\in Q} \lambda_q \sum_{x\in \cX} P(x) q(x) - \log(Z) \\
%     = \sum_{q\in Q} \lambda_q  q(P) - \log(Z)
% \end{align*}
% \end{proof}

% We use the following  notation:
% Let the private dataset be denoted by $P$ with $n$ records.  $\cX$ is the data universe, and $Q=\{q_1, \ldots, q_m\}$ a set of statistical queries.
% %
% We denote $U$ as the uniform distribution over the domain $\cX$.
% %
% For a given error tolerance $\gamma$, our goal is to find a synthetic dataset $D$ such that for any $q\in Q$ we had $|q(P) - q(D) |\leq \gamma$. 
% A way to cast the query release problem is as a constrained optimization problem:

% %
% \begin{align}\label{eq:opt}
%     \text{minimize:}\quad &\diver{D \parallel U} \\
%     \notag
%     \text{subject to: }\quad & \forall_{q\in Q}\quad \left|q(P) - q(
%     D)\right | \leq \gamma,
%     \quad \forall_{x\in\cX}\quad D(x) \geq 0 ,  
%     \quad \sum_{x\in \cX} D(x) = 1
% \end{align}
% % 
% Here we show that
% \begin{theoremrep}
% Let $\Dprivbf$ be a dataset, then solving \ref{eq:opt} is equivalent to finding $\Dbf$ that minimizes $\sum_{x\in \cX} P(x) \log\pp{\frac{D(x)}{U(x)}}$.
% \end{theoremrep}
% \begin{proof}
% We can write the Lagrangian of \ref{eq:opt}:
% \begin{align*}
%     \cL = \diver{\Dbf \parallel \Ubf} + \sum_{q\in Q} \lambda_q \pp{{q(\Dprivbf)} - q(\Dbf)} 
%     + \mu\pp{\sum_{x } D(x) - 1}
% \end{align*}
% Minimizing $\cL$ with respect to $D(x)$:
% \begin{align*}
% 0 = \frac{\partial\cL }{\partial D(x)} = 
% \log\pp{\frac{D(x)}{U(x)}} + 1
% %
%  - \sum_{q\in Q_0} \lambda_q q(x)
%  + \mu \\ 
%  \implies
% % 
% D(x) = U(x) \exp\pp{\sum_{q\in Q} \lambda_q q(x) - \mu -1}
% \end{align*}
% After choose $\mu$ to satisfy a distribution we get
% \begin{align*}
%   D(x) = \frac{U(x)}{Z} \exp\pp{\sum_{q\in Q} \lambda_q q(x) } 
% \end{align*}
% where $Z = \sum_{x\in \cX} \exp\pp{\sum_{q\in Q} \lambda_q q(x) } $.
% Plugging into $\cL$ we get
% \begin{align*}
%       \cL &= \sum_{x\in \cX} D(x)\log\pp{\frac{D(x)}{U(x)}} + \sum_{q\in Q} \lambda_q \pp{q(\Dprivbf) - q(\Dbf) } \\ 
%       &= \sum_{x\in\cX} D(x) \pp{\sum_{q\in Q} \lambda_q q(x)} 
%       - \log(Z)
%       + \sum_{q\in Q} \lambda_q\pp{q(\Dprivbf) - q(\Dbf)}  \\
%       %
%       &=  \pp{\sum_{q\in Q} \lambda_q q(\Dbf)} 
%       - \log(Z)
%       + \sum_{q\in Q} \lambda_q\pp{q(\Dprivbf) - q(\Dbf) - \gamma} \\
%       %
%       &=  
%       - \log(Z)
%       + \sum_{q\in Q} \lambda_q q(\Dprivbf) \\
%         &=  
%         \sum_{x\in \cX} P(x) \log\pp{\frac{D(x)}{U(x)}} \tag{claim \ref{claim:I}}
%       %
% \end{align*}
% It follows that solving \ref{eq:opt} is equivalent to minimizing $ \sum_{x\in \cX} P(x) \log\pp{\frac{D(x)}{U(x)}}$.
% \end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Iterative Projection
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Iterative Projection} 
Now we discuss how to solve \ref{eq:opt} using the \emph{Iterative Projection } technique. 
\input{docs/algos/pep}
% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Write here the result }
% %  initialization\;

% \textbf{Input:}
% Number of iterations $T$, linear queries $Q = \{q_1, \ldots, q_m\}$,  and answers $\{\ahat_1, \ldots, \ahat_m \}$ \\
% \textbf{Objective:} Minimize $ \diver{\Dbf\parallel \Ubf} $  such that  $\forall_{i \in [m]} \quad q_i(\Dbf) =  \ahat_i$ \\
% Initialize $\Dbf_0$ to be the uniform distribution over $\cX$ \\ 
% \For{ $t = 1, \ldots T$}{
%   \textbf{Choose:} $i \in [m]$  with 
%   $i \leftarrow \argmax_{j}  \pp{\ahat_i - q_i(\Dbf_t) }$. \\
%   %
%   \textbf{Update:} For all $x\in\cX$,  $D_{t+1}(x) \leftarrow D_{t}(x) e^{-\alpha q_i(x)}$, 
%   where 
%   $-\alpha = \ln\left( \frac{\ahat_i (1-q_i(\Dbf_t)) }{(1-\ahat_i) q_i(\Dbf_t)} \right)$.
%   %
%  }
%   \textbf{Output:}  $\Dbf_T$
%  \caption{Iterative Projection}
%  \label{alg:IP}
% \end{algorithm}

% \begin{figure}
%     \centering
% \includegraphics[width=\textwidth]{figures/temp.png}
%     % \includegraphics{}
%     \caption{A plot of $\frac{\Lexp_{T+1}}{\Lexp_T}$ for different values of $q(D)$ and $q(\Dprivbf)$}
% \label{img:LTplot}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
% Suppose that we run 
Let $\Dbf_t$ be the output of algorithm \ref{alg:IP} running on query set $Q$ with answer vector $\ahat$. Let 
 $e_t := \max_{q\in Q}| \ahat_i - q_i(\Dbf_t)|$ be the error after $t$ iterations. Then $e_t$ converges to zero with a rate of $O(\tfrac{1}{t})$.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Let $\Dbf_0 = \Ubf$ be the initial distribution.  Let $q_t$ be the query selected in round $t$ and 
note that $q_t$ is selected to maximize the distance to $\Dbf_t$, in other words 
\begin{align*}
    q_{t+1} \leftarrow \argmax_{q\in Q} \min_{\Dbf: q(\Dbf) = q(\Dprivbf)} \diver{\Dbf \parallel \Dbf_t}
\end{align*}

Given a query $q_t\in Q$, the constraint optimization problem during time $t$ is given by 
%
\begin{align}\label{eq:IP}
    \text{minimize:} &\quad\diver{\Dbf\parallel \Dbf_t} \\  
    \notag
   \text{subject to: }&\quad  q_t(\Dprivbf) - q_t(\Dbf) = 0 ,
    \quad
    \forall_{x\in \cX}  D(x) \geq 0, 
    \quad
    \sum_{x\in \cX} D(x) = 1
\end{align}



% We can write the Lagrangian of \ref{eq:IP}: 
Let $\Dbf\in \mathbb{R}^{|X|}$ and $\lambda \in \mathbb{R}$. Then the Lagrangian of \ref{eq:IP} is:
%
\begin{align}\label{eq:lagrangian}
    \cL(D, \lambda) = \diver{\Dbf\parallel \Dbf_t} + \alpha_t \left(q_t(\Dprivbf) -  q_t(\Dbf)   \right) + \mu\left(\sum_{x\in\cX}D(x) - 1\right) 
\end{align}
%
Taking the partial derivative with respect to $D(x)$ we have 
%
\begin{align}\label{eq:dellagrangian}
    \frac{\partial \cL(\Dbf, \lambda)}{\partial D(x)} =
    \ln\pp{\frac{D(x)}{D_t(x)}} + 1 
    -  \alpha_t  q_t(x) + \mu =0
\end{align}
%
Solving \ref{eq:dellagrangian} for $D(x)$ we get
\begin{align}\label{eq:updatestep}
    D(x) = D_t(x)e^{\alpha_t q_t(x) - 1 - \mu} 
    = D_t(x)\frac{e^{\alpha_t q_t(x)} }{Z_t} 
\end{align}
where $\mu$ is chosen to satisfy the constraint $\left(\sum_{x\in\cX}D(x)\right) = 1$ and $Z_t$ is a regularization factor.
%
%
Plugging \ref{eq:updatestep} into \ref{eq:lagrangian} we get:
\begin{align*}\label{eq:lagrangian}
    \cL(D, \lambda) &= \diver{\Dbf \parallel \Dbf_t} + \alpha_t \left(q_t(\Dprivbf) -  q_t(\Dbf) \right) + \mu\left(\sum_{x\in\cX}D(x) - 1\right) \\
    %
    &= \sum_{x} D(x) \log\pp{ \frac{D(x)}{D_t(x)}} + \alpha_t \left(q_t(\Dprivbf) -  q_t(\Dbf) \right)
        \\ 
     &= \sum_{x} D(x) \alpha_t q_t(x) - \log(Z_t)+ \alpha_t \left(q_t(\Dprivbf) -  q_t(\Dbf) \right) \\ 
      %
    &= - \log(Z_t)+ \alpha_t q_t(\Dprivbf)  \tag{Since    $\alpha_t q_t(\Dbf) =  \sum_{x} D(x) \alpha_t q_t(x)$} \\
    %
    &= - \log(Z_t)+ \log\pp{ e^{ \alpha_t q_t(\Dprivbf)}}   \\
        %
    % &= - \log(Z_t)+ \sum_{x\in\cX} P(x)\log\pp{\frac{D(x)}{D_t(x)}}
        % \\ 
    &= -\log\pp{\frac{Z_t}{\exp\pp{\alpha_t q_t(\Dprivbf)}}}
\end{align*}
where $Z_t = \sum_{x\in\cX} D_t(x)e^{\alpha_t q_t(x)} = e^{\alpha_t}q_t(\Dbf_t) + \qbar_t(\Dbf_t)$
%
Since the $q_t$ is chosen to maximize $\cL$, that corresponds to choosing $\alpha_t$ to maximize $\cL$. Equivalently, we  can say that that $\alpha_t$ is chosen to minimize


\begin{align}\label{eq:minimizationproblem}
\frac{Z_t}{e^{\alpha_t q_t(\Dprivbf)}} = 
  \frac{\sum_{x\in\cX}D_t(x)\exp\pp{\alpha_t q_t(x)}}{ \exp\pp{\alpha_t q_t(\Dprivbf)}}
    = \sum_{x\in\cX} D_t(x) \exp\pp{\alpha_t \pp{q_t(x) - q_t(\Dprivbf)}}
\end{align}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% To find the value 
We can define the unnormalized distribution on round $T$ as
\begin{align*}
    \Dhat_T(x) =D_1(x) \exp\pp{\sum_{t=1}^{T-1} \alpha_t \pp{q_t(x) - q_t(\Dprivbf)}}
\end{align*}
where $\Dhat_1(x) = \tfrac{1}{|\cX|}$.
Note that we can recover $\Dbf_T$ from $\Dhatbf_T$ if we let $\Zhat_T = \sum_{x\in\cX}\Dhat_T(x) $ then $D_T(x) = \frac{\Dhat_T(x)}{\Zhat_T}$.
%
Then we define the exponential loss on round $T$ as:
\begin{align*}
    \Lexp_T = \sum_{x\in\cX} \Dhat_T(x)
\end{align*}

To show  that \iter tries to minimize $\Lexp_T$ consider $\Lexp_{T+1}$:
\begin{align}
   \label{eq:lossexp}
   \Lexp_{T+1} =  \sum_{x\in\cX} \Dhat_{T+1}(x) 
%   \notag
   &=  \sum_{x\in\cX} \Dhat_T(x)\exp\pp{\alpha_t\pp{q_t(x)-q_t(\Dprivbf)}}
%   &= \frac{ \sum_{x\in\cX} \Dhat_T(x)\exp\pp{\alpha_t\pp{q_t(x)}} }
%   {\exp\pp{\alpha_t q_t(\Dprivbf)}}
\end{align}

Note that 
\begin{align}
   \label{eq:lossexpratio}
   \frac{\Lexp_{T+1}}{\Lexp_T} =  \sum_{x\in\cX} D_T(x)\exp\pp{\alpha_t\pp{q_t(x)-q_t(\Dprivbf)}}
%   &= \frac{ \sum_{x\in\cX} \Dhat_T(x)\exp\pp{\alpha_t\pp{q_t(x)}} }
%   {\exp\pp{\alpha_t q_t(\Dprivbf)}}
\end{align}

% We see that \eqref{eq:minimizationproblem} and \eqref{eq:lossexp} are very similar except for the unnormalized distribution. However since $\Dhat_T(x) \propto D_T(x)$ this two optimization problems are equivalent. To see this note that dividing equation \eqref{eq:lossexp} by the normalization factor $Z_T$ does not change the minimum of the function.
Therefore, we can see that $q_t, \alpha_t$ are selected to minimize  \eqref{eq:lossexpratio}. We can write
%
%
\begin{align}\label{eq:LTplusone}
\frac{\Lexp_{T+1}}{\Lexp_T} &=
% \Lexp_{T+1} &= 
\min_{\alpha}
    \left[
    e^{\alpha (1-q(\Dprivbf))}q(\Dbf_{T}) + e^{-\alpha q(\Dprivbf)}(1-q(\Dbf_{T})) 
    \right] 
\end{align}

Differentiating w.r.t $\alpha$ and setting $0= \frac{\partial \Lexp_{T+1}}{\partial \alpha}$ we get
\begin{align*}
%  0= \frac{\partial \Lexp_{T+1}}{\partial \alpha}
%     &= 
%         e^{\alpha (1-q(\Dprivbf))}q(\Dbf_{T})\pp{1-q(\Dbf_T)}
%         -
%         e^{-\alpha q(\Dprivbf)}(1-q(\Dbf_{T})) q(\Dprivbf)   \\
% \implies
 e^{\alpha (1-q(\Dprivbf))}q(\Dbf_{T})\pp{1-q(\Dbf_T)}
&= e^{-\alpha q(\Dprivbf)}(1-q(\Dbf_{T})) q(\Dprivbf) \\  
 e^\alpha &=\frac{q(\Dprivbf)(1-q(\Dbf_T)}{(1-q(\Dprivbf) q(\Dbf_T)}
\end{align*}



\color{gray}

 Plugging in $e^\alpha$ into \eqref{eq:LTplusone}  we get
%
%
\begin{align*}
\frac{\Lexp_{T+1}}{\Lexp_T}
    % \Lexp_{T+1} 
    &=  \pp{\frac{q(\Dprivbf)(1-q(\Dbf_T))}{(1-q(\Dprivbf)) q(\Dbf_T)}}^{ (1-q(\Dprivbf))}q(\Dbf_{T}) 
    + \pp{\frac{(1-q(\Dprivbf)) q(\Dbf_T)}{q(\Dprivbf)(1-q(\Dbf_T))}}^{ q(\Dprivbf)}(1-q(\Dbf_{T}))
\end{align*}


The function $\frac{\Lexp_{T+1}}{\Lexp_T}$ looks complicated but can plot it for some values of $q(\Dbf_{T})$ and $q(\Dprivbf)$. In figure \ref{img:LTplot}, we can see that, for a fixed value of $q(\Dbf)$, the function $\Lexp_{T+1}$ appears to behave like a parabola.



% \paragraph{Error Analysis}




Let $q_1, \ldots, q_T$ be the sequence of queries selected. We have that $q_t \leftarrow \argmax_{q\in Q} \pp{q(\Dprivbf) - q(\Dbf_t)}$.
From figure \ref{img:LTplot} , we get the following inequality for any $q_{t+1}\in Q$ and any round $t+1$:
%
\begin{align}\label{eq:gapI}
    \pp{ | q_{t}(\Dprivbf) - q_{t}(\Dbf_{t}) | }^2  
    \leq
    1 - \frac{\Lexp_{t+1}}{\Lexp_{t}} 
\end{align}

How can we interpret equation \eqref{eq:gapI}? I think this means that ITER reduces ratio of the exponential function. Therefore we can think of ITER as decreasing the exponential potential function by multiplicative factors, as suppose to MWEM which reduces the KL potential by an additive factor.





Let $e_t := \max_{q\in Q}| q(\Dprivbf) - q(\Dbf_t)| $ . Then, using inequality \eqref{eq:gapI} we have
\begin{align}
    \prod_{t=1}^T \frac{\Lexp_{t+1} }{L_t}
    &\leq \prod_{t=1}^T (1-e_{t}^2) \\ 
%
     \frac{\Lexp_{T+1} }{L_0}
    &\leq \prod_{t=1}^T (1-e_{t}^2)
\end{align}



Under the assumption that $e_t < e_t'$ for $t>t'$:
Suppose that $e_t \geq \alpha$ for all $t\leq T+1$ and $e_t< \alpha$ for all $t>T+1$, and $\Lexp_0 = 1$ we get
$\Lexp_{T+1} \leq \prod_{t=1}^T (1-\alpha^2)= (1-\alpha^2)^T$. Therefore 
\begin{align}\label{eq:alphaerror}
    \alpha^2 &\leq 1-\pp{\Lexp_{T+1}}^{1/T} \\ 
    &\leq \log\pp{\frac{1}{\Lexp_{T+1}}}\frac{1}{T}
    = -\frac{\log\pp{\Lexp_{T+1}} }{T} && \text{using inequality \eqref{ineq:nthroot}}
\end{align}

\end{proof}



\color{black}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% See figure \ref{fig:curve} to visualize equation \eqref{eq:alphaerror}. We can see that it resembles the empirical error of ITER in figure \ref{fig:iter}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/curve.png}
%     \caption{Curve of $1-\pp{0.4}^{1/T}$}
%     \label{fig:curve}
% \end{figure}


% {\color{blue} I think the $\log(|\cX|) $ term will should up in $\Lexp_{T+1}$ after we add privacy.}





% If we can prove \eqref{eq:gapI} then we can write 
% %
% %
% \begin{align}
%     % \notag
%     \label{eq:gapII}
%     \pp{ q_{T+1}(\Dprivbf) - q_{T+1}(\Dbf_{T+1})  }^2  
%     &\leq \Lexp_{1} - \sum_{t=1}^T  \pp{q_t(\Dprivbf) - q_t(\Dbf_t)}^2  
%     % &=1 - \sum_{t=1}^T \max_{q} |q(\Dprivbf) - q(\Dbf_t)| 
% \end{align}
% the term $\Lexp_1$ is some constant that depends on the data..

% We can consider a base case where we show that if $\Lexp_{T+1} = \Lexp_T$ then $q(\Dbf_{T})=q(\Dprivbf)$ for all $q$:



% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/MWConvADULTsmall.png}
%     \includegraphics[width=0.45\textwidth]{figures/ITERConvADULTsmall.png}
%     \caption{Comparing convergence of MW vs ITER: ADULT-small workload is 32.}
%     \label{fig:iter}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/MWConvADULTmed.png}
%     \includegraphics[width=0.45\textwidth]{figures/ITERConvADULTmed.png}
%     \caption{Comparing convergence of MW vs ITER: ADULT-medium workload is 32.}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/MWEMConvADULTsmall.png}
%     \includegraphics[width=0.45\textwidth]{figures/PITERConvADULTsmall.png}
%     \caption{Comparing convergence of MWEM vs PITER: ADULT-small workload is 32.}
%     \label{fig:piter}
% \end{figure}



% \paragraph{Convergence}
% We define a set of distributions $\cP = \{ \pbf:  q(\pbf) = q(\Dprivbf) \quad \text{ for all } q\in Q \}$ that contain all distributions that satisfy the constrains of equation \ref{eq:opt}. 

% Let $\Dhatbf_t$ be an unnormalized distribution defined as $\Dhat_t(x) = \exp\pp{\sum_{i=1}^t \alpha_i (q_i(x) - q_i(P))}$. Note that can always recover the normalized distribution:for any $x\in\cX$ we have $D_t(x) = \frac{\Dhat_t(x)}{\sum_{x\in\cX} \Dhat_t(x)}$.
% The we define the exponential loss on round $t$ as $L_t = \sum_{x\in\cX}\Dhat_t(x)$. We want to show that if $\Dhatbf_t$ is at the minimum of $L_t$ then $\Dbf_t\in \cP$.
 
 

% let $L_{t+1} = \min_{\q,\alpha} \sum_{x\in\cX} \Dhat_t(x) \exp\pp{\alpha \pp{\q(x) - \qI{P}}}$ be  loss function after one update. We can write $L_{t+1}$ as
% %
% \begin{align*}
%     L_{t+1} &= \min_{\q,\alpha}\sum_{x:\q(x)=1} \Dhat_t(x) \exp\pp{\alpha \pp{1- \qI{\Dprivbf}}}
%   +\sum_{x:\q(x)=0} \Dhat_t(x) \exp\pp{-\alpha \qI{\Dprivbf}} \\
%   %
%   &= \min_{\q,\alpha}\pp{ \exp\pp{\alpha (1-\qI{\Dprivbf})}\qI{\Dhatbf_t}
%   + \exp\pp{-\alpha \qI{\Dprivbf}}(1-\qI{\Dhatbf_t})}
% \end{align*}

% For any $\q\in Q$, using calculus we can solve $\frac{\partial L_{t+1}}{ \partial \alpha} = 0$ to get the value of $\alpha$:

% % 
% \begin{align*}
%   \frac{\partial L_{t+1}}{ \partial \alpha} &= \exp\pp{\alpha (1-\qI{\Dprivbf})}\qI{\Dhatbf_t}(1-\qI{\Dprivbf})
%   - \exp\pp{-\alpha \qI{\Dprivbf}}(1-\qI{\Dhatbf_t})\qI{\Dprivbf} \\
% \implies 0    &= \exp\pp{\alpha}\qI{\Dhatbf_t}(1-\qI{\Dprivbf})
%   - (1-\qI{\Dhatbf_t})\qI{\Dprivbf}\tag{Multiply by $e^{\alpha \qI{\Dprivbf}}$}
% \end{align*}
% %
% Setting $\frac{\partial L_{t+1}}{ \partial \alpha} = 0$ we get
% \begin{align*}
%     e^\alpha = \frac{(1-\qI{\Dhatbf_t}) \qI{\Dprivbf}}{\qI{\Dhatbf}(1-\qI{\Dprivbf})}
% \end{align*}

% Next suppose that $L_{t+1} = 1$ then 

% \begin{align*}
%      &e^{\alpha (1-\qI{\Dprivbf})}
%      \qI{\Dhatbf_t}
%   + e^{-\alpha \qI{\Dprivbf}}
%   (1-\qI{\Dhatbf_t}) = 1 \\
%      &e^{\alpha }
%      \qI{\Dhatbf_t}
%   + 
%   (1-\qI{\Dhatbf_t}) = e^{\alpha \qI{\Dprivbf}} \\
% %   \implies&     \exp\pp{\alpha (1-\qI{\Dprivbf})}\qI{\Dhatbf_t}
% %   + \exp\pp{-\alpha \qI{\Dprivbf}}(1-\qI{\Dhatbf_t})
% %   - \qI{\Dhatbf} - (1-\qI{\Dhatbf}) = 0 \\
% %     \implies&    
% %     %
% %     \exp\pp{\alpha }\qI{\Dhatbf_t}
% %   + (1-\qI{\Dhatbf_t})
% %   - \exp\pp{\alpha \qI{\Dprivbf}}\qI{\Dhatbf} - \exp\pp{\alpha \qI{\Dprivbf}}(1-\qI{\Dhatbf}) = 0
% \end{align*}


==> docs/unused/ITER_MC_queries.tex <==

\section{Iterative Projection for Convex Minimization (CM) Queries}
Let $\Theta\subset \mathbb{R}^d$ be a convex set.
Consider a class of convex loss functions $L = \{\ell:\Theta\times\cX\rightarrow \mathbb{R} \}$. For any $\ell\in L$ the corresponding CM query  has the form:
%
\begin{align*}
q_\ell(D) = \argmin_{\theta} \sum_{x\in\cX} D(x) \ell(\theta;x)
\end{align*}
%
An example of a class of convex queries is defined the $\ell_2$-regularized square loss functions :
\begin{align*}
L^{\text{SqLoss}} = \{ \ell_\beta:\Theta\times\cX\rightarrow \mathbb{R} : \beta\geq 0 \}
\text{, where }\quad 
    \ell_\beta(\theta, x, y) 
    = (\langle \theta, x\rangle - y)^2 + \beta \|\theta\|_2^2
\end{align*}

For any $\ell_\beta\in L^{\text{SqLoss}}$, the corresponding convex query is:
    $q_{\ell_\beta}(D) := \argmin_\theta \sum_{(x,y)\in \cX}D(x,y)\ell_\beta(\theta, x, y)$.

%
The error of a synthetic dataset $D$ on loss $\ell$ and query $q_\ell$ with respect to a private dataset $\Dpriv$ is.
\begin{align}\label{eq:cqerror}
\qerror(\Dpriv, D) =  \left|\ell( q_\ell(D), \Dpriv ) - \min_{\theta}\ell(\theta, \Dpriv)\right|
\end{align}

%
The goal is to find a dataset $D$ s.t. $\max_{\ell \in L} \qerror(\Dpriv, D)$  is small.

In order to use the Iterative projection technique we must be able to formulate the program as an optimization problem with linear constraints. 
When solving for linear queries the objective is to find a $D$ that minimizes $\abs{q(D)- q(\Dpriv)}$, which defines a linear constrain for every linear query $q$.

In the case of CM queries, the objective \cref{eq:cqerror} does not define a linear constraint that we can feed into the iterative projection algorithm. However, we can use the optimally conditions of convex problems that the gradient must be zero at the optimal point. 


Let $\theta_{\ell, D}$ be the minimum solution when the data is $D$, i.e. 
 $\theta_{\ell, D} = \argmin_{\theta} \ell(\theta, D)$. Suppose that, on round $t$, we sample a loss function $\ell_t$ with high error as in \cref{eq:cqerror} and let $\thetatil_{\ell_t, \Dpriv} =\theta_{\ell_t, \Dpriv} + \text{Lap}(1/\epsilon')$ be a noisy measurement of the minimum solution on the real data. 

By the optimality condition we expect $\nabla_\theta \ell_t(\thetatil_{\ell_t, \Dpriv}, \Dpriv) \approx 0_{d} $, therefore we would want our synthetic dataset $\Dsync$ to satisfy the following constraint  
%
\begin{align}\label{eq:gradconst}
\nabla_\theta \ell_t\left(\thetatil_{\ell_t, \Dpriv}, \Dsync\right) = 0_{d}
\end{align}
%
Let $i\in [d]$ be a gradient coordinate. Then we can write 

$$ \sum_{x\in\cX} \Dsync(x) \nabla_\theta \ell_t\left(\thetatil_{\ell_t, \Dpriv}, x \right) = 0 $$


\begin{algorithm}[H]
\SetAlgoLined
% \KwResult{Write here the result }
 Let $d$ be the dimension of the parameter space $\Theta$.
 Given a private dataset $\Dpriv$, set of convex queries $L = \{\ell: \Theta\times \cX\rightarrow \mathbb{R} \}$. \\
 Let $D_0$ be a dataset sampled from the uniform distribution. \\ 
 \For{$t = 0 \ldots (T-1)$}{
  Choose: $\ell_t \in L$ using the Exponential Mechanism with score $\qerror(\Dpriv, D_t)$, as in \cref{eq:cqerror} \\
%   $$\pr{q_t = q} \propto \exp\left(\frac{|q(D) - q(D_{t})|}{2\epsilon}\right)$$
  %
%   Add $q$ to $\Qprev$.\\
  Get noisy measurement: let $\theta_t = \argmin_\theta \ell_t(\theta, \Dpriv) + \text{Lap}(1/\varepsilon)$. \\
  \tcp{Apply IP: Note that $\nabla_{\theta_t} \ell_t(\theta_t, D) = 0$ defines $d$ linear constraints}
  Choose:  $D_{t+1} = \text{arg}\min_{D} \diver{D\parallel U} $, such that for all $i\leq t$, $\nabla_{\theta_i} \ell_i(\theta_i, D) = 0$ 
 }
  Output weighted dataset $\{D_T\}$\\
 \caption{Iterative projection for Convex Queries}
\end{algorithm}

==> docs/unused/ITER_unnormed.tex <==

\section{Iterative Projection for Linear Queries}
\textbf{ Changing to unnormalized distributions}


Try the query projection algorithm from \cite{nikolov2013geometry} with the Iterative projection protocol. That is first the the noisy answers $\qtil(\Dprivbf) = q(\Dprivbf) + \text{Gaussian}(\rho)$. Then use IP to find a dataset that matches the answers $\hat{a}$.

Let $\cX$ be a data universe, $Q$ a set of statistical queries, where every query maps an element of $\cX$ to the set $\{-1, 1\}$.
%
We can construct a query set that is close under negation, let $\Qbar$ be the set that contains $Q$ and  is close under negation: For any $q\in Q$ we have that $q\in \Qbar$ and  $\bar{q} \in \Qbar$ where $\bar{q}(x) = -q(x)$ for any $x\in\cX$. Finally, we denote the private dataset by $\Dprivbf$ . 



We denote $\one$ as the one vector over the domain $\cX$.
Absent the constraint of privacy the objective is to find a dataset $D$  that solves the following program:
%
\begin{align}\label{eq:opt}
    \text{minimize:}\quad &\diverunnormed{\Dbf \parallel \one} \\
    \notag
    \text{subject to: }\quad & \forall_{q\in Q}\quad q(\Dpriv) =  q\pp{\Dbf},
    \quad \forall_{x\in\cX}\quad D(x) \geq 0 ,  
\end{align}
%
where for two two vector $\pbf,\qbf \in \mathbb{R}_{+}^m$, $\diverunnormed{\pbf \parallel \qbf}$ is the unnormalized relative entropy.

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

Next we device a differentially private algorithm that approximates the objective of \cref{eq:opt}. 
The algorithm  operates over $T$ rounds and on each round solves an optimization problem similar to \cref{eq:opt}. 
That is, on every round $t$, we formulate a modify version of \cref{eq:opt} and use Iterative Projection to solve it.
%
On round $t$, we have a set of $t$ queries $Q_t = \{q_1, \ldots, q_t \}$ that were selected using a private mechanism and define $t$ constraints.
For every query $q\in Q_t$, let $\qtil(\Dprivbf) = q(\Dprivbf) + Lap(1/\varepsilon)$ be the private answer to query $q$. By the properties of the Laplace mechanism we have $|\qtil(\Dprivbf) - q(\Dprivbf) |\leq  \frac{\log(1/\beta)}{\varepsilon}$, with probability at least $1-\beta$. 
%
Let  $\gamma = \frac{\log(1/\beta)}{\varepsilon}$ and $\alpha$ be the accuracy tolerance of the optimization, then our algorithm solve the following constraint optimization problem using iterative projection: 
%

\begin{align}\label{eq:privopt}
    \text{minimize:}\quad &\diverunnormed{\Dbf \parallel \one} \\
    \notag
    \text{subject to: }\quad & \forall_{q\in \Qbar} \quad   \qtil(\Dprivbf) \leq q(\Dbf) + \gamma + \alpha,
    \quad
    \forall_{x\in \cX} \quad  D(x) \geq 0, 
\end{align}
%
Note that for any $q\in Q$, if \cref{eq:privopt} is satisfied for all queries in $\Qbar$ then we have 
\begin{align*}
    \qtil(\Dprivbf) - q(\Dbf) \leq \gamma + \alpha \text{ and }
    -\qtil(\Dprivbf) + q(\Dbf) \leq \gamma + \alpha
\end{align*} 
therefore we have that with high probability $|q(\Dprivbf) - q(\Dbf)| \leq \alpha$, which is what we want.



%
We need to find a $\Dbf_{t+1}$ that solves \cref{eq:privopt}.
To solve \cref{eq:privopt} we use iterative projection: For $K$ rounds, on round $k \in [K]$, we find $\Dbf_{k+1}$ by first picking one constraint $q_k \in Q_t$ and finding the closes distribution to $\Dbf_k$ that satisfies $q$. Here is the objective: 
%
\begin{align}\label{eq:privoptIP}
    \text{minimize:}\quad &\diverunnormed{\Dbf \parallel \Dbf_k} 
    & \quad \text{subject to: }\quad & \quad \qtil_k(\Dprivbf) \leq q_k(\Dbf)  + \gamma + \alpha,
    \quad
    \forall_{x\in \cX} \quad  D(x) \geq 0, 
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lagrangian
We can write the Lagrangian of \cref{eq:privoptIP}: 
Let $\Dbf \in \mathbb{R}^{|X|}$ and $\lambda \in \mathbb{R}$. Then the Lagrangian of \cref{eq:privopt} is:
%
\begin{align}\label{eq:lagrangian}
    \cL(\Dbf, \lambda) &= \diverunnormed{\Dbf\parallel \Dbf_k} + \lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha \right)  \\ 
    \notag
    &=\sum_{x\in\cX} \pp{ D(x) \log\pp{\frac{D(x)}{D_k(x)}} + D_k(x)-D(x)}
    + \lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha  \right)
\end{align}
%
Taking the partial derivative with respect to $D(x)$ we have 
%
\begin{align}\label{eq:dellagrangian}
    \frac{\partial \cL(D, \lambda)}{\partial D(x)} =
    \ln\pp{\frac{D(x)}{D_k(x)}} 
    - \lambda  q_k(x) =0
\end{align}
%
Solving \cref{eq:dellagrangian} for $D(x)$ we get
\begin{align}\label{eq:updatestep}
    D(x) = D_k(x) e^{\lambda q_k(x)} 
\end{align}
%
%
Plugging \cref{eq:updatestep} into \cref{eq:lagrangian} we get:
\begin{align*}
    \cL(D, \lambda) &= \diverunnormed{\Dbf\parallel \Dbf_k} +
    \lambda \left(\qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha  \right)  \\
    %
    &=\sum_{x\in\cX} \pp{ D(x) \log\pp{\frac{D(x)}{D_k(x)}} + D_k(x)-D(x)}
        +\lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha  \right) \\ 
    &=\sum_{x\in\cX} \pp{ D(x) \log\pp{\frac{D_k(x)e^{\lambda q_k(x)} }{D_k(x)}} + D_k(x)-D(x)}
        +\lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha  \right) \\ 
    &=\sum_{x\in\cX} \pp{ D(x) \pp{\lambda q_k(x)} + D_k(x)-D(x)}
        +\lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha  \right) \\ 
    &= \lambda\sum_{x\in\cX}D(x) q_k(x) +  \sum_{x\in\cX} \pp{ D_k(x)-D(x)}
        +\lambda \left( \qtil(\Dprivbf) - q(\Dbf) - \gamma - \alpha \right) \\ 
    &=  \sum_{x\in\cX} \pp{ D_k(x)-D(x)}
        +\lambda \left( \qtil_k(\Dprivbf) - \gamma -\alpha \right) \tag{ because 
        $\sum_{\in\cX}D(x) q_k(x) = q_k(\Dbf)$} \\ 
    &=  \sum_{x\in\cX} D_k(x) - \sum_{x\in\cX} \pp{ D_k(x)e^{\lambda q_k(x)}}
        +\lambda \left( \qtil_k(\Dprivbf) - \gamma - \alpha \right)  \\ 
%  &=  \sum_{x\in\cX}D_k(x) \pp{1 - e^{-\lambda q_k(x)}}
%         -\lambda \left( A_{q_k} + \gamma \right)  \\ 
\end{align*}

Therefore we have to choose $\lambda $ to minimize $Z(\lambda) = \sum_{x\in\cX} \pp{ D_k(x)e^{\lambda q_k(x)}} - \lambda \left( \qtil_k(\Dprivbf) - \gamma -\alpha \right) $


The next step is to find the optimal value of $\lambda$, therefore we need to calculate the derivative of $Z(\lambda) $ with respect to $\lambda$:
\begin{align*}
    \frac{\partial Z(\lambda)}{\partial \lambda} 
    &= \sum_{x\in\cX} D_k(x) e^{\lambda q_k(x)} q_k(x) - \qtil_k(\Dprivbf) + \gamma + \alpha \\ 
    %
    &= e^{\lambda}\sum_{x:q_k(x)=1} D_k(x) 
    - e^{-\lambda}\sum_{x:q_k(x)=-1} D_k(x) 
    - \qtil_k(\Dprivbf) + \gamma + \alpha \\ 
    %
    &= e^{\lambda}W_k^{+} (\Dbf_k)
    -e^{-\lambda}W_k^{-}(\Dbf_k)
    - \qtil_k(\Dprivbf) + \gamma + \alpha
    %
    %
    % &= e^{-\lambda} q_k(D_k)- A_{q_k} - \gamma \\ 
    % &= \frac{e^{-\lambda} q(D_k)}{\sum_{x\in\cX } D_k(x) e^{-\lambda q_k(x)} } - (\Atil_{q_k} + \gamma)\\
    % &= \frac{e^{-\lambda} q(D_k)}{e^{-\lambda} q_k(D_k) + \bar{q}_k(D_k) }- (\Atil_{q_k} + \gamma)
\end{align*}


Setting $\frac{\partial Z(D, \lambda)}{\partial \lambda}  = 0$, we can solve for $\lambda$

\begin{align*}
   e^{\lambda}W_k^{+} (\Dbf_k)
    -e^{-\lambda}W_k^{-}(\Dbf_k)
    - \qtil_k(\Dprivbf) + \gamma + \alpha = 0 \\ 
    %
    \implies
       e^{2\lambda}W_k^{+} (\Dbf_k)
       + e^{\lambda}\pp{\gamma + \alpha - \qtil_k(\Dprivbf) }
        -W_k^{-}(\Dbf_k) = 0 
% \implies        e^{2\lambda}W_k^{-}
% + e^{\lambda} (\qtil_k(\Dprivbf) + \gamma)
% -W_k^{+}  = 0 \\ 
    %
    % -\lambda = \log\pp{\frac{A_{q_k} + \lambda}{q_k(D_k)}}
\end{align*}
Solving for $e^\lambda$ we get 
\begin{align}\label{eq:learningrate}
    e^\lambda = \frac{- (\gamma + \alpha - \qtil_k(\Dprivbf)) + 
    \sqrt{
        \pp{\gamma + \alpha - \qtil_k(\Dprivbf)}^2 + 4 W_k^{+} (\Dbf_k)W_k^{-}(\Dbf_k)
        }
    }{W_k^{+} (\Dbf_k)}
\end{align}
% Next we show that $q_k(D_{k+1}) \approx \Atil_{q_k}$.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% EM+IP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithm}

The algorithm uses iterative projection to find a dataset that matches the answers of all queries with high error, which were found by calling the EM. 


\newcommand{\Qprev}{Q_{\mathrm{prev}}}
\begin{algorithm}[H]
\SetAlgoLined
% \KwResult{Write here the result }
%  initialization\;
 Given a private dataset $\Dprivbf$, 
 A set of linear queries $Q$, the set of negated queries $\Qbar$, accuracy tolerance $\alpha$ \\
 Let $\Dhatbf_0 \leftarrow \one$. \\ 
 \For{$t = 0 \ldots (T-1)$}{
 \tcp{Exponential mechanism:}
  Choose $q_t$ using the Exponential Mechanism with score: 
  $\pr{q_t = q} \propto \exp\left(\frac{q(\Dprivbf) - q(\Dhatbf_{t})}{2\epsilon}\right)$\\
  %
%   Add $q$ to $\Qprev$.\\
  Let $\qtil_t(\Dprivbf) \leftarrow q_t(\Dprivbf) + \text{Lap}(1/\varepsilon)$. \\ 
  \tcp{Apply iterative projection:}
  Choose 
  $\Dhatbf_{t+1} \leftarrow \text{arg}\min_{\Dbf} \diverunnormed{\Dbf\parallel \one} $  such that  $\forall_{i\leq t}\quad  \qtil_i(\Dprivbf) \leq q_i(\Dbf) + \gamma + \alpha$
 }
  Output dataset $\Dhatbf_T$\\
 \caption{ITEREM (Primal) (Iterative Projection + EM )}
 \label{alg:ITER}
\end{algorithm}


Given a history of queries, ITER can find a dataset with error close to zero on the given queries. The algorithm is not efficient since it has to keep track of the whole data domain which can be very large in high dimension data regimes. However, this algorithm can be adapted 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% IP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
\SetAlgoLined
% \KwResult{Write here the result }
%  initialization\;

\textbf{Input:} A set of linear negated queries $\Qbar$,  and noisy measurements $\{\qtil(\Dprivbf) \}_{q\in \Qbar}$ \\
\textbf{Objective:} Minimize $ \diverunnormed{D\parallel \one} $  such that  $\forall_{q\in \Qbar} \quad  \qtil(\Dprivbf) \leq q(D)  + \gamma + \alpha$ \\

Initialize $\Dsync_0 \leftarrow \one$ to be the uniform distribution over $\cX$ \\ 
Initialize $i \leftarrow 0$ \\  
 
\While{error is more than $\gamma+\alpha$}{
  \textbf{Choose:} $q \in \Qbar$  with 
  $q \leftarrow \argmax_{q\in\Qbar}  \pp{\qtil(\Dprivbf) - q(\Dsync_i) }$. \\
  %
  \textbf{Update:} For all $x\in\cX$,  
  $$\Dsync_{i+1}(x) \leftarrow \Dsync_{i}(x) \exp\pp{\lambda_i q(x)}$$ 
  where 
  $\lambda_i$ is set as in \cref{eq:learningrate}. \\
  %
  \textbf{Update:} index $i \leftarrow i + 1$. \\
 }
  \textbf{Output:}  $D_i$
 \caption{Iterative Projection}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis}
\begin{enumerate}
    \item Have a data dependent bound for \cref{alg:ITER}.
    \item Do a follow the regularized proof for \cref{alg:ITER}. (\href{https://lucatrevisan.github.io/40391/lecture12.pdf}{FTRL Notes})
\end{enumerate}
In this section we analyze \cref{alg:ITER}.
In this section we let $\Dhat_t$ denote the un-normalized distribution of \iter during round $t$, and
 define the exponential loss function to be 
$$L_t = \sum_{x\in\cX} \Dhat_{t}(x) - \lambda_{t-1}\pp{\qtil_{t-1}(\Dprivbf) -\gamma-\alpha}$$


The analysis goes as follows:
\begin{itemize}
    % \item Show that if $q_t(\Dpriv) - q_t(D_t)$ is small the $L_{t+1} - L_t$ will be small.
    \item Show that when $L_{t+1} - L_t < C$ then  $q_t(\Dpriv) - q_t(\Dhatbf_t) <\approx C$.
\end{itemize}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% theorem:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}Given a private dataset $\Dprivbf$ and a set of linear queries $Q$.
One round $t$, let $\Dhatbf_t$ be the synthetic dataset produced by \iter. 
If $L_{t} - L_{t+1} < C$ then for all $q\in Q$, with probability at least $1-\beta$ we have
%
\begin{align*}
q(\Dprivbf) - q(\Dhatbf_t) \leq
    \mathrm{polylog}\pp{C, \log(1/\beta)}
\end{align*}
\end{lemma}

\begin{proof}

For this proof we assume that $q(x) \in \{-1,1\}$ for all $x\in\cX$.

Let
$$L_t = \sum_{x\in\cX} D_{t}(x) - \lambda_{t-1}\pp{\qtil_{t-1}(\Dprivbf) - \gamma - \alpha}$$

be the exponential loss of \cref{alg:ITER}. 
% We will see  \cref{alg:ITER} chooses a $q\in Q$ to maximize $L_t$ and $\alpha_t$ to minimize $L_t$. Therefore we can write loss function after one update as:
and 
$$L_{t+1} =\min_{q, \lambda} \sum_{x\in\cX} D_{t}(x)e^{\lambda q(x)} - \lambda\pp{\qtil(\Dprivbf) - \gamma - \alpha}$$. 

For all $q\in Q$, let $W^{+}_{q}(\Dhatbf) = \sum_{x: q(x)=1}\Dhat(x)$  and $W^{-}_{q}(\Dhatbf) = \sum_{x: q(x)=-1}\Dhat(x)$. We can write


\begin{align*}
    L_{t} = W^{+}_{q}(\Dhatbf_t) + W^{-}_{q}(\Dhatbf_t)- \lambda_{t-1}\pp{\qtil_{t-1}(\Dprivbf) - \gamma - \alpha}
\end{align*}
and 
\begin{align*}
    L_{t+1} &= e^{\lambda }W^{+}_{q} (\Dhatbf_t)
    + e^{  -\lambda} W^{-}_{q}(\Dhatbf_t) - \lambda\pp{\qtil(\Dprivbf) - \gamma - \alpha} \\ 
    &=  - (\gamma + \alpha - \qtil(\Dprivbf)) + 
    \sqrt{
        \pp{\gamma + \alpha - \qtil(\Dprivbf)}^2 + 4 W_{q}^{+} (\Dbf_t) W_q^{-}(\Dbf_t)
        } \\
    &+ \frac{W_{q}^{+}(\Dhatbf_t)W_q^{-}(\Dhatbf_t)}{- (\gamma + \alpha - \qtil(\Dprivbf)) + 
    \sqrt{
        \pp{\gamma + \alpha - \qtil(\Dprivbf)}^2 + 4 W_{q}^{+} (\Dbf_t)W_q^{-}(\Dbf_t)}
    } \\ 
    &  - \lambda\pp{\qtil(\Dprivbf) - \gamma - \alpha} \\ 
    %
    %
    &=\pp{- (\gamma + \alpha - \qtil(\Dprivbf)) + 
    \sqrt{
        \pp{\gamma + \alpha - \qtil(\Dprivbf)}^2 + 4 W_{q}^{+} (\Dbf_t)W_q^{-}(\Dbf_t)
        }}^2
    \pp{ 1 + W_{q}^{+}(\Dhatbf_t)W^{-}_{q}(\Dhatbf_t)} \\
    &- \lambda\pp{\qtil(\Dprivbf) - \gamma - \alpha} 
\end{align*}
\end{proof}

==> docs/unused/PITER.tex <==



% \paragraph{Bounding error:} We want to bound
% \begin{align*}
% \max_{q\in Q}
% q(\Dprivbf) - q(\Dbf)
% =
% \max_{q\in Q}
% \sum_{x \in \cX} q(x)\Dpriv(x) - \sum_{x\in \cX} q(x)D(x)
% =\max_{q\in Q}\mathbb{E}_{x\sim \Dprivbf}
%     \left[ 
%     q(x) - q(x)\frac{D(x)}{\Dpriv(x)}
%     \right]
% \leq \max_{q\in Q} \mathbb{E}_{x\sim \Dpriv}
%     \left[ 
%     q(x)\pp{1 - \frac{D(x)}{\Dpriv(x)}}
%     \right]
% \end{align*}



% \paragraph{Proof strategy}
% Let $\cP$ be a set such that $\cP = \{ p : \sum_{x\in \cX} p(x)q(x) = \widetilde{q(P)}  \text{ for } q\in Q\}$.
% We want to show that the sequence of distributions converges to the set that includes $P$. If want to find out if minimizing the exponential losses
% \begin{align*}
%  L_t =    \sum_{x\in\cX} D_t(x)
% \end{align*}
% is equivalent to solving $\argmin_{D\in \cP} \diver{D\parallel \one} $.



==> docs/unused/inequalities.tex <==
\begin{inequality}\label{ineq:nthroot}
Let $a\in (0,1)$ and $T$ be a positive integer, then
    $1-a^{1/T}\leq \frac{\log(\tfrac{1}{a})}{T}$
\end{inequality}
\begin{proof}
Do proof later. Use Lauren series.
\end{proof}


\begin{inequality}
Let $x,y\in (0,1)$ then the following holds:
\begin{align*}
    (x-y)^2 \leq 1 -\pp{ 
    \pp{\frac{y(1-x)}{(1-y)x}}^{1-y}x
    + \pp{\frac{(1-y)x}{y(1-x)}}^{y}(1-x)
    }
\end{align*}
\end{inequality}
\begin{proofsketch}
See figure \ref{img:LTplot}
\end{proofsketch}

==> docs/unused/methods_public_old.tex <==
\section{Extending to \textit{PAP} setting}

Incorporating prior information from public data has shown to be a promising avenue for private query release \cite{bassily2020private, liu2021leveraging}. Therefore in this section, we extend \pep and \gem to the problem of \textit{public-data-assisted private (PAP)} \citep{bassily2020private} query release, in which our differentially private algorithms have access to public data that are free of privacy concerns.

\peppub. Like in \citet{liu2021leveraging}, we extend \pep by making two changes: (1) we maintain a distribution over the public data domain and (2) we initialize the approximating distribution to that of the public dataset. Therefore like \pmwpub, \peppub also restricts $\cD$ to distributions over the public data domain and initializes $D_0$ to be the public data distribution.

\gempub. To adapt \gem to utilize public data, we again initialize $D_0$ to a distribution over the public dataset. However because in \gem, we implicitly model any given distribution using a generator $G$, we must first train without privacy (i.e., without using the exponential and Gaussian mechanisms) a generator $G_{\textrm{pub}}$, to minimize the $\ell_1$-error over some set of queries $\hat{Q}$. Note that in most cases, we can simply let $\hat{Q} = Q$ where $Q$ is the collection of statistical queries we wish to answer privately. \gempub then initializes $G_0$ to $G_{\textrm{pub}}$ and proceeds with the rest of the \gem algorithm.

\subsection{Overcoming limitations of \pmwpub and \peppub.} \label{sec:pub_limitations}

We describe limitations of \pmwpub and \peppub by providing two example categories of public data that these algorithms fail to utilize effectively. In addition, we describe how \gempub overcomes such limitations in both scenarios.
 
\textbf{Public data with insufficient support.} 
We first discuss the case in which the public dataset has an insufficient support, which in this context means the support has high \textit{best-mixture-error} \citep{liu2021leveraging}. Given some support $S$, the \textit{best-mixture-error} can be defined as
%
\begin{align*}
    \min_{\mu \in \Delta(S)} 
    \max_{q\in Q}
    \left|
    q\pp{D} - 
    \sum_{x \in S} \mu_x  q(x)
    \right|
\end{align*}
%
where $\mu \in \Delta(S)$ is a distribution over the set $S$ with $\mu_x \ge 0$ for all $x\in S$ and $\sum_{x\in S} \mu_x = 1$. In other words, the \textit{best-mixture-error} approximates the best possible error that can be achieved by reweighting some support, which in this case means that both \peppub and \pmwpub cannot achieve max errors lower that this value. While \citet{liu2021leveraging} offer a solution for filtering out poor public datasets ahead of time using a small portion of the privacy budget, \peppub and \pmwpub cannot be run effectively if no other suitable public datasets exist. \gempub however avoids this issue altogether because unlike the aforementioned methods, which cannot be run without restricting the size of $\cD$, \gempub can utilize public data without restricting the distributional family it can represent (since both \gem and \gempub compactly parametrize any distribution using a neural network).

\textbf{Public data with incomplete data domains.} Next we consider the case in which the public dataset only has data for a subset of the attributes found in the private dataset. We note that as presented in \citet{liu2021leveraging}, \pmwpub cannot handle this scenario. One possible solution (for both \pmwpub and \peppub) is to augment the public data distribution by assuming a uniform distribution over all remaining attributes missing in the public dataset. However, while this may work in cases where only a few attributes are missing, the missing support grows exponentially in the dimension of the missing attributes. In contrast, \gempub can still make use of public data that is missing attributes found in the private dataset. In particular, we can pretrain a generator $G$ on queries over just the attributes found in the public dataset. Again, \gempub avoids the computational intractability of \pmwpub and \peppub in this setting since it parametrizes its output distribution with $G$.

==> docs/unused/mwem_update.tex <==
\subsection{\mwem loss function derivation} \label{sec:mwemupdate}

% Fix round $t$, let $\eta_t = \atil_t - \qtil_t(D_{i-1})$ be the learning rate during round $t$ and $D_{t-1}$ be the distribution from the previous round.
Then \mwem's loss function is:
%
\begin{align}\label{eq:mwemloss}
    % D_{t} \leftarrow 
    \cL^{\text{mwem}}(D, \Qtil_t, \Atil_t)
    % \argmin_{D\in \Delta(\cX)} =
    = \eta_t \sum_{x\in \cX} D(x) \qtil_i(x) 
    + \sum_{x\in\cX} D(x) \log\pp{\frac{D(x)}{D_{t-1}(x)}}
\end{align}
%
% \swcomment{there is a mismatch in the main text. it was relative entropy w.r.t. the uniform distribution}
% \gv{I have the old version of this. I can switch it if you want or update the main text to match this version. }


The optimization problem becomes $D_t = \argmin_{D\in \Delta(\cX) } \cL^{\text{mwem}}(D, \Qtil_t, \Atil_t)$. 
The solution $D$ is some distribution, which we can express as a constraint $\sum_{x\in \cX} D(x) = 1$. Therefore, this problem is a constrained optimization problem.
To show that \eqref{eq:mwemloss} is the \mwem's true loss function,
we can write down the Lagrangian as:
\begin{align*}
        \cL
    % \argmin_{D\in \Delta(\cX)} =
    = \eta_t \sum_{x\in \cX} D(x) \qtil_i(x) 
    + \sum_{x\in\cX} D(x) \log\pp{\frac{D(x)}{D_{t-1}(x)}}
    + \lambda \pp{\sum_{x\in \cX} D(x) - 1}
\end{align*}

Taking partial derivative with respect to $D(x)$:
%
\begin{align*}
      \frac{\partial \cL}{\partial D(x) }  
    % \argmin_{D\in \Delta(\cX)} =
    =  \eta_t \qtil_i(x) 
    + 1 + \log \frac{D(x)}{D_{t-1}(x)} 
    + \lambda
\end{align*}
Setting $ \frac{\partial \cL}{\partial D(x) }   = 0$ and solving for $D(x)$:
\begin{align*}
D(x) = 
D_{t-1}(x)\exp\pp{-1 - \lambda - \eta_t \qtil_i(x)   }
\end{align*}

Finally, the value of $\lambda $ is set such that $D$ is a probability distribution:

\begin{align*}
D(x) = 
\frac{
D_{t-1}(x) \exp\pp{- \eta_t\qtil_t(x)   }
}
{
\sum_{x\in\cX}D_{t-1}(x)\exp\pp{ - \eta_t \qtil_t(x) }
}
\end{align*}
This concludes the derivation of \mwem's loss function.
\swcomment{did you miss a sum over $t$ in the exp?}

==> figures/all_errors/sensitivity_trick.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/all_errors/sensitivity_trick.png}
    \caption{
    Performance for \pep with the $k$-way marginal sensitivity trick (Appendix \ref{appx:sensitivity_trick}) on ADULT (reduced) (workloads=35), evaluated on $3$-way marginals with privacy budgets $\varepsilon \in \{ 0.1, 0.15, 0.2, 0.25, 0.5, 1 \}$ and $\delta = \frac{1}{n^2}$. The \textit{x-axis} uses a logarithmic scale. Results are averaged over $5$ runs, and error bars represent one standard error.
    }
    \label{fig:all_errors_sensitivity_trick}
\end{figure}
